Wi-Fi All-Channel Analyzer

In this paper, we present WACA, the first system to simultaneously measure the energy in all 24 Wi-Fi channels that allow channel bonding at 5 GHz with microsecond scale granularity. With WACA, we perform a first-of-its-kind measurement campaign in areas including urban hotspots, residential neighborhoods, universities, and a sold-out stadium with 98,000 fans and 12,000 simultaneous Wi-Fi connections. The gathered dataset is a unique asset to find insights otherwise not possible in the context of multi-channel technologies like Wi-Fi. To show its potential, we compare the performance of contiguous and non-contiguous channel bonding using a trace-driven framework. We show that while non-contiguous outperforms contiguous channel bonding's throughput, occasionally bigger by a factor of 5, their average throughputs are similar.

==> sections/11ax.tex <==
%\subsection{802.11ax Constraints}
\label{sec:11ax}

Here, we consider additional constraints imposed by 802.11ax  on channel bonding. Namely, 802.11ax defines three modes of channel bonding, each of which restrict channel bonding to a subset of channels \cite{tgax2019draft}. For example, U-NNI-1 and U-NNI-2 restrict channel bonding groups to 
%EK looks great but takes too much space
\begin{comment}
\begin{align*}
    \mathcal{C}_{\mathcal{B}_\text{1\&2}} &= \{ \{1,2\}, \{3,4\}, \{5,6\}, \{7,8\},\\
    &\{1,2,3,4\}, \{5,6,7,8\}, \{1,...,8\}\}
\end{align*}
\end{comment}
$\mathcal{C}_{\mathcal{B}_\text{1\&2}} = \{ \{1,2\}, \{3,4\}, \{5,6\},$
$\{7,8\}, \{1,2,3,4\}, \{5,6,7,8\}, \{1,...,8\}\}$
so that (for example) a 40 MHz bonded channel that combines channels 2 and 3 is not allowed. Notice that we do not use the IEEE 802.11 channel indices (e.g., 36,40,44,...) in the example above for ease of exposition. While reducing throughput when only a single BSS bonds, such restrictions can reduce fragmentation if multiple BSS's bond. Moreover, such restrictions simplify implementation. Thus, here we study the cost of 802.11ax's channelization restrictions when a single BSS bonds and compare to the non-restricted cases explored this~far.

\textbf{Static Channel Bonding (SCB):}  employs a \emph{fixed} channel width and therefore must always use the same set of channels. It can be viewed as an``all-or-nothing'' policy: for example, if static channel bonding uses 8 consecutive basic channels (160 MHz), it must wait until all 8 channels are free in order to  transmit using the entire 160 MHz. Although simple to implement, it is vulnerable to excessive deferral while waiting for all channels to become available.  

\textbf{Dynamic Channel Bonding (DCB)}: picks the largest available set of contiguous basic channels found free subject to both the primary channel being included  and the total set of channels being an allowed set under the restrictions such as above. For example, if channel 4 is selected as a primary channel, dynamic channel bonding allows bonded transmissions with channels $\{3,4\}$, $\{1,2,3,4\}$, or $ \{1,...,8\}$, as well as single channel transmission on channel 4. Other combinations such as $\{4,5\}$ are not permitted.

\textbf{Preamble Puncturing (PP)}: allows puncturing wide channels, i.e., aggregating non-contiguous basic  channels. Even though the total channel is still subjected to the above channelization constraints, preamble puncturing is more flexible than dynamic channel bonding since it enables non-contiguous channel combinations, provided the primary channel is included \cite{tgax2019draft,qu2019survey}. For example, a transmission using primary channel 3 could transmit on 60 MHz using channels $\{1,3,4\}$, which would be a punctured subset of $\{1,2,3,4\}$. Nonetheless,  not every combination of punctured channels is allowed in the standard. For instance, $\{1,3\}$ is not permitted.

Observe that both static and dynamic channel bonding are restricted special cases of contiguous channel bonding studied previously, whereas preamble puncturing is a restricted special case of non-contiguous channel bonding. 

%EK thinks the reader will not understand this
% Sergio: OK, let's skip it from the paper. I plan to detail the code in GitHub once it is accepted.
% \begin{comment}
% Contiguous and non-contiguous policies assess the spectrum occupancy of non-primary channels just at the end of the backoff $t_\text{BO}$, i.e., $\gamma_{t_\text{BO}} = \neg x_{t_\text{BO}}$, where $x_{t_\text{BO}}$ is a binary vector determining the occupancy of each \textit{basic} channel at $t_\text{BO}$, whereas \textit{802.11ax} policies select $\mathcal{T}_{t_\text{BO}}$ according both to a channelization $\mathcal{C}$ and to the spectrum status during the previous $T_\text{PIFS}$. Namely, \textit{basic} channels are now considered as usable only if they were found idle during the entire $T_\text{PIFS}$ before the backoff terminated. Consequently, $\gamma_{t_\text{BO},c} = \big((\sum_{t=t_\text{BO}-T_\text{PIFS}}^{t_\text{BO}}x_{t,c}) > 0 : 0, 1\big)$.
% \end{comment}	

\sloppy
Here, we compare the throughput of both the (non-restricted) contiguous and non-contiguous polices with the three 802.11ax policies, all using selection of the best primary channel. Figure~\ref{fig:11ax_ratios} shows the resulting 802.11ax throughput normalized to the unrestricted case for the respective category of contiguous or non-contiguous.

	\begin{figure}[t!]
		\centering
		\includegraphics[width=0.34\textwidth]{11ax_ratios.eps}
		\caption{Best primary throughput ratio of the IEEE 802.11ax policies with respect to contiguous and non-contiguous channel bonding.}
		\label{fig:11ax_ratios}
	\end{figure}


First, observe that 802.11ax static channel bonding suffers severe throughput degradation compared to contiguous channel bonding. Namely, the desirable simplicity of static channel bonding comes with a high performance cost. For example, under heavy load, static channel bonding only obtains 39\% of the throughput compared to contiguous channel bonding, indicating that too much time is spent deferring to realize significant gains from wide channels. Moreover, static channel bonding also encounters poorly performing outliers, well below the mean. For example, the 1\%-percentile performance is less than 10\% for medium and high loads, even less than single channel allocation.

Second, comparing 802.11ax dynamic channel bonding to contiguous channel bonding (middle bars), we observe that it achieves 87\% to 81\% of the average throughput of contiguous channel bonding for low and high load respectively, with 1\%-percentiles over 65\% for any load regime. 

Finally, comparing 802.11ax preamble puncturing to non-contiguous channel bonding (right set of bars),  the former obtains 96\% to 94\% of the throughput of the latter in low and high load respectively. Further, throughput differences are kept smaller also in the most divergent scenarios, reaching 1\%-percentiles over 77\% for all the loads. 
	
\textit{Finding}: IEEE~802.11ax channelization restrictions have a modest throughput cost compared to non-restricted. For example, standard-compliant preamble puncturing obtains over 90\% of the throughput of (non-restricted) non-contiguous channel bonding. Unfortunately, the simplest standard policy, static channel bonding, performs quite poorly. 


==> sections/correlation.tex <==
\subsection{Inter-Channel Occupancy Correlation} \label{sec:correlation}

When a transmitter finds its primary channel available for transmission and attempts to bond channels, it aims to find secondary channels available. Thus, correlation among channel occupancies can be expected to help channel bonding performance. Here we study the spectral correlation of the best primary channel with other channels and compute the mean correlation coefficient as
\begin{equation}
	\begin{split}
	\xi &= \sum_{p \in \mathcal{B}, p \neq p^*} \rho(p^*,p)/ \big(|\mathcal{B}|-1\big),\text{ with}\\
	& \rho(p^*,p) = \frac{\mathbb{E}[(p^* - \mu_{p^*})(p - \mu_{p})]}{\sigma_{p^*}\sigma_{p}}
	\end{split}
\end{equation}
where $\mathcal{B} \in \{\mathcal{B}_\text{1\&2},\mathcal{B}_\text{2c}\}$, thus $|\mathcal{B}|=8$, $\rho(p^*,p)$ is the Pearson correlation coefficient of the temporal occupancy of channels $p^*$ and $p$, as a function of the means, $\mu_{p^*}$ and $\mu_{p}$, and  standard deviations, $\sigma_{p^*}$ and $\sigma_{p}$, of channel $p^*$ and $p$, respectively. Notice that this assessment of spectral correlation by simultaneously measuring all channels is achieved for the first time by \sys.


\begin{figure}[ht]
		\centering
		\includegraphics[width=0.42\textwidth]{correlation_distribution_cdf.png}
		\caption{Distribution and empirical CDF of the best primary channel correlation $\xi$.}
		\label{fig:correlation_distribution_cdf}
\end{figure}


Figure~\ref{fig:correlation_distribution_cdf} shows both the distribution of $\xi$ vs. mean occupancy $\bar{o}_\mathcal{B}$ and the empirical cumulative distribution function (CDF) of $\xi$. We observe that $\xi$ ranges approximately from -0.10 to 0.60, so we define three correlation levels for ease of analysis: low ($\xi \leq 0.1$), medium ($0.2 \leq \xi < 0.4$), and high ($\xi \geq 0.5$). While we find that most of the periods (62\%) fall inside the low correlation range, 17\% of them present medium or higher correlation, indicating a significant amount of correlated epochs. A key origin of correlation among channels in the data set may be that the APs are already using channel bonding. Indeed, even though the dataset does not provide header information, some subsets of traces have multiple contiguous channels having almost identical busy/idle evolution. This suggests that channel bonding was employed during some portions of the measurement campaign.

% I would not indicate STATIC channel bonding since both dynamic and static would perform the same under fully idle spectrum


\begin{figure}[ht]
	\centering
	\begin{subfigure}{0.46\textwidth}
		\centering
		\includegraphics[width=\textwidth]{img/results_correlation_3_categories_low.eps}
		\caption{Low-correlation periods.}
		\label{fig:results_correlation_low}
	\end{subfigure}
	%
	\begin{subfigure}{0.46\textwidth}
		\centering
		\includegraphics[width=\textwidth]{img/results_correlation_3_categories_med.eps}
		\caption{Medium-correlation periods.}
		\label{fig:results_correlation_med}
	\end{subfigure}
	%
	\begin{subfigure}{0.46\textwidth}
		\centering
		\includegraphics[width=\textwidth]{img/results_correlation_3_categories_high.eps}
		\caption{High-correlation periods.}
		\label{fig:results_correlation_high}
	\end{subfigure}
	\caption{Evolution of the best-primary normalized throughput vs. correlation. We use transparencies at the points to highlight denser regions.}
	\label{fig:results_correlation}
\end{figure}
	

%Figure \ref{fig:results_correlation} shows  throughput given selection of the best primary channel, with the sub-figures highlighting intervals with low correlation ($\xi < 0.2$) and high correlation ($\xi > .5$). First, observe that the low-correlation figures indicate that the data largely follows this low correlation sub-sampled data set. In other words, the measured channel occupancies show minimal inter-channel correlation. However, the high-correlation figures indicate that for the sub-sampled high correlation periods, more pronounced throughput gains could be realized, both for contiguous and non-contiguous channel bonding, with the gains for contiguous being the highest.

Figure \ref{fig:results_correlation} shows  throughput given selection of the best primary channel, with the sub-figures highlighting intervals with low, medium, and high correlation. We observe that most of the measured channel occupancies show minimal inter-channel correlation. However, the figures for periods of medium and high correlation indicate that with higher correlation among channel occupancy, the lower performance periods are increasingly avoided, especially for contiguous channel bonding. Interestingly, this effect holds regardless of the mean occupancy $\bar{o}_\mathcal{B}$.

\textit{Finding}: There are significant periods (17\%) presenting medium to high correlation among channel occupancies. Such periods improve the performance of channel bonding regardless of the load. This can provide a hint as to what ideally would happen if multiple BSS's employ channel bonding, since channel bonding itself creates channel-occupancy correlation.


==> sections/depriving.tex <==
\subsection{How Much Are Others Hindered?}

%This far, we have evaluated how much throughput is gained from channel bonding. However, when one BSS gains access to multiple channels, nearby BSS's operating on other channels will have to defer. 

When other BSS's defer to a channel bonder, it will  add to their channel access latency and could decrease their throughput. Here, we study how much all other BSS's are hindered due to channel bonding and introduce a bandwidth deprivation metric $\omega$ as the aggregate bandwidth that would have been active (i.e., was being used by neighbor BSS's) during the transmissions of the channel bonding BSS. This metric can serve as an upper bound to how much others are hindered by viewing that all of these attempts by other BSS's would be lost vs. deferred. 
%
More formally, let
	\begin{equation}
	\omega = \frac{\big(\sum_{f=1}^{n_f}\sum_{t\in \mathcal{T}_f}\sum_{c\in \mathcal{B}_{\text{tx},f}} x_{t,c}\big) bT_\text{s}}{T_\text{per}},
	\end{equation}
	where $n_f$ is the number of frames transmitted, $\mathcal{T}_f$ is the set of consecutive temporal samples used for transmitting frame $f$, $\mathcal{B}_{\text{tx},f}$ is the set of channels used for transmitting frame $f$, $T_\text{s}$ is the duration of a temporal sample (\SI{10}{\micro\second}), $b = 20$ MHz is the bandwidth of a basic channel, and $T_\text{per} = \SI{100}{ms}$ is the observation duration. We normalize by $T_\text{per} = \SI{100}{ms}$ rather than the transmission time of each policy to provide a fair comparison. That is, $\omega$ represents how much raw bandwidth is deprived to surrounding BSSs in absolute terms [MHz], without considering how many transmissions are performed by each policy.
	
Figure~\ref{fig:results_bw_prevention} shows the distribution (boxplot) of the bandwidth deprivation in MHz and Mbps for every  primary channel using  the occupancy categories defined in \S\ref{sec:cont_noncont}. In order to estimate the corresponding data rate, we assume that all occupied samples are comprised of 20-MHz data frames transmitted at MCS 9. The figure illustrates the intrinsic consequences of bonding channels without considering how the others might use the spectrum during the transmission. Namely, a channel bonder may find that most channels are free at backoff termination, thus subsequently occupying most (or all) of them. However, it may occur that right after starting the transmission, external activity appears in some  of the channels being used, thus hindering surrounding BSS's.

\begin{figure}[t!]
		\centering
		\includegraphics[width=0.38\textwidth]{results_bw_prevention.eps}
		\caption{Distribution of bandwidth and data rate lost for other BSS's for every primary channel.}
		\label{fig:results_bw_prevention}
\end{figure}

% cont similar to non-cont
Second, we observe that the differences in bandwidth deprivation for non-contiguous vs. contiguous channel bonding are quite modest, even when non-contiguous channel bonding achieves higher throughput. The key reason is that most high occupancy periods concentrate activity in some 20 MHz channels, often leaving at least one 20 MHz channel idle during nearly the entire period. In contrast to contiguous, non-contiguous channel bonding can always realize small throughput gains by bonding those idle channels regardless of the primary channel allocation.
% Outliers
Also, despite the low average impact, there are multiple outliers in which the bandwidth lost by other BSS's is significantly higher than average, thus manifesting the worst-case external effect.

Finally, we can ask if channel bonding is simply a zero-sum-game: do the gains of a bonding BSS simply subtract from other BSS's throughput? To address this question, we assess whether the average throughput gained by channel bonding exceeds the worst-case prevented transmissions by other BSS's, using  single channel transmission as a baseline. Thus, we define the ratio
\begin{equation}
    \kappa_\pi = \frac{\bar{\Gamma}_\pi - \bar{\Gamma}_\text{SC}}{\bar{\omega}_\pi - \bar{\omega}_\text{SC}}, 
\end{equation}
where $\bar{\Gamma}_\pi$ and $\bar{\Gamma}_\text{SC}$ are the mean throughput of policy $\pi$ and SC, and $\bar{\omega}_\pi$ and $\bar{\omega}_\text{SC}$ are the corresponding mean throughput deprivation. A value $\kappa_\pi = 1$ would indicate that the trade-off between the bonding gain and external throughput deprivation is actually a zero-sum-game, whereas $\kappa_\pi > 1$ would indicate net gains. The results indicate that both contiguous and non-contiguous channel bonding yield substantial net gains over all occupancy regimes. Specifically, $\kappa_\text{CO} =  95.2, 68.9, 49.4$ for contiguous, and $\kappa_\text{NC} = 91.9, 65.7, 45.5$ for non-contiguous, under low, medium, and high occupancy regimes, respectively. 

\textit{Finding}:  In the worst case, a channel bonding BSS can hinder neighbors by 100's of Mb/sec. However, the \emph{average} hindrance is quite low and neighbors can defer instead of not transmitting to reduce the impact. Moreover, the data rate gained by bonding far exceeds the worst-case data rate lost by neighbors, since neighbors are not always backlogged during bonding epochs.


==> sections/hidden.tex <==
\subsection{The Hidden Cost of Hidden Nodes}
\label{sec:hidden}

\sergio{If we keep this, remove all the correlation stuff and include a brief description of the simulator.}

Here, we continue our study of potential detrimental effects of channel  bonding by considering the case of hidden nodes. We again impose a worst-case scenario on the measurements as follows: channel access occurs as previously with contention occurring on the primary channel and  channel bonding adding channels according to availability and the policy, contiguous or non-contiguous. However, here we reconsider the measured activity that occurs during the bonded transmission. While in the previous subsection, we considered that the other BSS's would have deferred, here, we consider that other BSS's are hidden from the bonded transmission and still transmit and result in frame loss. Thus, this scenario considers that the RTS/CTS mechanism is not used or fails and disallows capture effects in which the higher signal-to-noise ratio receiver correctly decodes, e.g., \cite{SJ-Lee-capture}. Thus, in these two ways, this experiment provides an empirical upper bound as to the damage that hidden terminals could do to a channel bonded transmission.

In particular, we assume that a frame $f$ is lost if temporal samples are found active in any of the channels used for transmitting $f$. Specifically, $f$ is lost if the following expression holds, 
	\begin{equation} \label{eq:loss}
	\sum_{t\in \mathcal{T}_f}\Big(\big(\sum_{c\in \mathcal{B}_{\text{tx},f}}x_{t,c}\big) \geq 1 : 1,0\Big) \geq \alpha |\mathcal{T}_f|, 
	\end{equation}
	where $\mathcal{T}_f$ is the set of consecutive temporal samples required for transmitting frame $f$, and the term $\sum_{c\in \mathcal{B}_{\text{tx},f}} x_{t,c}$ denotes the number of occupied channels at time $t$. We apply a factor $\alpha = 0.01$ to exclude spurious noise as cause of loss. Thus, we avoid for instance losing an entire frame when just a single temporal sample was found active during the transmission. 

	\begin{figure}[t!]
		\centering
		\begin{subfigure}{0.34\textwidth}
			\centering
    		\includegraphics[width=\textwidth]{img/hinder_norm_throughput.eps}
    		\caption{Hindering.}
    		\label{fig:hinder_norm_throughput}
		\end{subfigure}
		%
		\begin{subfigure}{0.34\textwidth}
			\centering
    		\includegraphics[width=\textwidth]{img/hidden_norm_throughput.eps}
    		\caption{Hidden terminals.}
    		\label{fig:hidden_norm_throughput}
		\end{subfigure}
		\caption{Distribution of the normalized best primary throughput.}
		\label{fig:results_hinder_hidden}
	\end{figure}
	
%Figure~\ref{fig:hidden_norm_throughput} depicts the throughput under this hidden-terminal scenario.
Figure~\ref{fig:hinder_norm_throughput} and Figure~\ref{fig:hidden_norm_throughput} depict the throughput distribution under hindering (without hidden terminals) and hidden-terminal scenarios, respectively. First, observe that throughput is significantly reduced in comparison to the case with no hidden terminals. For example, for contiguous channel bonding in high load, mean throughput gains over single-channel transmission are reduced from $5.2\times$ to $2.6\times$~(50\%). 

Second, there are significant  periods where channel bonding results in extremely low performance, even for low occupancy values. In fact, there are scenarios in which single-channel access outperforms bonding (blue areas where $\hat{\Gamma}^* < 1$ in the figure). In particular, single channel outperforms contiguous channel bonding in  18\%, 8\% and 8\% of the cases for low, medium and high occupancy, respectively. Even worse, single channel outperforms non-contiguous channel bonding in  38\%, 14\%, and 15\% of cases respectively. This illustrates that external traffic patterns may lead to accentuated chances of incurring collisions, thus impairing the performance of the channel bonder.

Third,  due to its more aggressive nature, non-contiguous channel bonding performs slightly worse than contiguous both in terms of average throughput and how often it is  outperformed by single channel transmission. This, together with the fact that contiguous performs similarly on average to non-contiguous without hidden terminals, indicates that gains provided by non-contiguous can be relatively small considering its greater risk and more complex design.

Finally, also in contrast to Figure~\ref{fig:hinder_norm_throughput},  Figure~\ref{fig:hidden_norm_throughput} indicates that the decaying trend of mean normalized best-throughput with load when neighbors defer does not hold with hidden terminals. Indeed, we observe a slight increase of the normalized best-throughput as the occupancy increases as fewer bonding opportunities also diminish the risk of collisions. 
	
\sloppy
\textit{Finding}: While channel bonding outperforms single-channel transmission in most cases, it is vulnerable to hidden node interference, with non-contiguous channel bonding being impacted the most. To avoid the aforementioned worst-case throughput penalties, nodes can use RTS/CTS, implement capture (to better receive even while a hidden terminal transmission overlaps in time), or increase channel sensing sensitivity, i.e., reduce the threshold for sensing channel activity to reduce the frequency of hidden terminal transmissions. 


==> sections/markov.tex <==
\subsection{A Markov Model for Channel Occupancy?}

%In \S\ref{sec:correlation}, we found that even though channels could be considered to be uncorrelated on average since activity is expected to be normally from separate BSS's, traces exhibited a significant amount of epochs of inter-channel occupancy correlation. With this experiment, we aim at pointing out the importance of capturing inter-channel correlation by comparing the original traces against two simple models.
%
In particular, we first consider a Markov model that characterizes each channel as an independent two state (occupied, not occupied) Markov chain with exponential holding times for each state. We compute the mean transition rates (and hence mean occupied and not-occupied time) for each channel from the traces.  We then compare performance between the parameter-matched Markov model and the actual traces. As a baseline, we also consider a \emph{uniform i.i.d.} model in which each epoch is occupied or not according to an i.i.d. Bernoulli distribution, with each channel again having the mean band occupancy matched from data. Our objective is not to develop a statistical occupancy model, but rather to study the extent to which simple models can or cannot characterize the behavior we observe.

We study below downlink throughput for these two models as compared to the traces when applying contiguous channel bonding. Since the throughput is impacted by the primary channel selection, we evaluate the selection of the 16 possible primary channels: 8 in sub-band $\mathcal{B}_{1\&2}$ and 8 in~ $\mathcal{B}_\text{2c}$.
	

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.48\textwidth]{img/synth_throughput_cb-cont.eps}
	\caption{Throughput vs. occupancy}
		\label{fig:synth_throughput}
\end{figure}
	
    Figure \ref{fig:synth_throughput} shows the raw throughput (considering every possible primary) of the original traces and the synthetic model-generated occupancy. While both models capture the general trend of throughput decaying with increasing occupancy, the difference between datasets is evident in the form of the scatter plots.
	
	% Norm throughput gain
	%Figure~\ref{fig:synth_norm_error} depicts the mean relative throughput error of the models with respect to the original traces. The i.i.d model has error of 38\%, 70\%, and 126\% for low, medium and high occupancy regimes, respectively. Unfortunately, although the Markov model also captures the mean on and off times for each channel, the errors are still quite significant, averaging 33\%, 58\%, and 62\% for low, medium and high occupancy regimes, respectively. \ewk{FIXME these numbers appear to be the maximum not the average. Max of all channels? Of all epochs?} \sergio{The maximum values previously included in Fig \ref{fig:synth_norm_error} referred to the maximum error resulting for a particular combination period and primary. Since I propose keeping the mean error bar chart without the max markers, I suggest including the following text.}
	Figure~\ref{fig:synth_norm_error} and Figure~\ref{fig:synth_norm_error_correlation} depict the mean relative error (MRE) of the models' throughput with respect to the original traces grouping by load and correlation regime, defined by the thresholds presented in \S\ref{sec:cont_noncont} and \S\ref{sec:correlation}, respectively. We observe that the i.i.d model is completely misleading with a mean error around 50\% for high loads and/or high correlation. Unfortunately, although the Markov model is able to capture the mean on and off times for each channel, we observe that the mean error is still significant (up to 16\% and 37\% on average for high load and high correlated periods, respectively). Worse, particular periods assessed through the Markov model lead to large errors up to 33\%, 58\%, and 62\% for low, medium and high occupancy regimes, respectively.

	% Why models are not accurate
	While we expected the higher relative errors to arise for high load periods, it is surprisingly critical the impact of not capturing correlation on both models. In fact, in contrast to the correlation distribution of the original traces shown in Figure~\ref{fig:correlation_distribution_cdf}, both models present a distribution similar to a delta function centered at $\xi=0$. Given that the original mean occupancy is kept for all the periods generated by the models, results suggest that missing correlation is the main cause of outraging the models' accuracy.
	
    \textit{Finding}: unfortunately, simple channel occupancy models severely underestimate the available gains for channel bonding. Thus, modeling occupancy behavior by introducing inter-channel correlation remains an important avenue for future work. Upon publication, all traces will be publicly available in order to foster this effort by the research community. 



==> sections/stadium.tex <==
\subsection{A Sold-Out Stadium} 
\label{sec:stadium}

Finally, we assess if channel bonding can provide throughput gains in areas with persistently high load over all channels. To study such a scenario, we deployed \sys in the press box of an urban stadium during a football game with over 98,000 spectators present (event and stadium not named to comply with double blinded reviewing; such information replaced with X). Figure~\ref{fig:fcb_location} shows a photograph of the setup. Measurements were taken on August 4, 2019, from 17:24 to 22:30 accounting for a total duration of 5~hours and 6 minutes. On that date, the
%Joan Gamper
\textit{X} trophy was held, which pitted the local club
%(Futbol Club Barcelona)
\textit{X} against the visiting club %(Arsenal Football Club)
\textit{X}.  Free Wi-Fi was provided to the audience through thousands of APs primarily installed beneath the seats.
	
	\begin{figure}[ht!]
		\centering
		
		\begin{subfigure}{0.22\textwidth}
			\centering
        	\includegraphics[width=\textwidth]{fcb_location_low.PNG}
    		\caption{\sys deployment.}
    		\label{fig:fcb_location}
		\end{subfigure}
		~
		\begin{subfigure}{0.225\textwidth}
			\centering
			\includegraphics[width=\textwidth]{fcb_traffic_square.png}
			\caption{Traffic evolution.}
			\label{fig:fcb_traffic}
		\end{subfigure}
		
		\begin{subfigure}{0.46\textwidth}
			\centering
			\includegraphics[width=1\textwidth]{fcb_occupancy_temporal.eps}
			\caption{Spectrum occupancy evolution.}
			\label{fig:fcb_occupancy_temporal}
		\end{subfigure}
		
		\caption{Wi-Fi activity at the \textit{X} stadium: a) \sys in \textit{X}'s press box, b) downlink and uplink Wi-Fi traffic evolution (source: \textit{X} stadium management), and c) spectrum occupancy evolution.}
		\label{fig:fcb_activity_plots}
	\end{figure}
	
We also obtained data from the stadium's network management team which indicated that up to 12,000 Wi-Fi clients were simultaneously connected. Downlink and uplink traffic is depicted in Figure~\ref{fig:fcb_traffic} and the spectogram in Figure~\ref{fig:fcb_occupancy_temporal}. Each slot in the spectogram represents the occupancy of each channel averaged in 1-second periods. We observe that most  channels were highly occupied during the measurements. Moreover, we can observe the users' behavior induced nonstationarity of the traces as the match progressed. Namely, while activity is always high, there is a notable reduction during  play (first and second half) compared to activity before, between halfs, and right after the game time.
We also observe that the majority of the channels are crowded most of the time with periods reaching mean band occupancy values $\bar{o}_\mathcal{B}$ rising up to 99\%. In fact, 22\% of the periods have $\bar{o}_\mathcal{B} > 0.8$. Nonetheless, we pose the question as to whether the remaining occupancy gaps can be exploited by channel bonding to boost aggregate throughput. 
%EK no need to state.
%We explore both contiguous and non-contiguous channel bonding.
% and partition results \sergio{WHAT ARE PARTITION RESULTS???} into the average occupancy of the epoch. 
	

                
\begin{figure}[ht]
\centering
\includegraphics[width=0.42\textwidth]{fcb_hinder.eps}
\caption{Gains for the bonding BSS.}
\label{fig:fcb_hinder}
\end{figure}
        
Figure~\ref{fig:fcb_hinder} shows normalized throughput under best primary channel selection when applying contiguous and non-contiguous channel bonding. Under loads exceeding 90\%,  both policies have throughput close to single channel transmission, indicating that there is simply minimal remaining margin for gain. Nonetheless, in transient epochs where load is low, both policies exploit throughput gains. For example, in the stadium during epochs of 20-30\% load, the gain over single channel throughput  is $3.69\times$ and $5.30\times$ for contiguous and non-contiguous respectively. In fact, we observe that non-contiguous significantly outperforms contiguous in a wide regime of ``non-extreme'' loads given the heterogeneous activity distribution over channels. For example, at 40-50\% average occupancy, contiguous channel bonding has average throughput gain of $2.38\times$ whereas non-contiguous has $3.97\times$, a gain of 67\%.

% Recall that for the non-stadium experiments in Figure \ref{fig:hinder_norm_throughput}, the gains during epochs of 20-30\% load (considered inside ``high'' load for the urban scenarios) were $5.19\times$ and $5.34\times$ for contiguous and non-contiguous bonding. Comparing to the stadium, non-contiguous channel bonding performs remarkably similarly  (5.30 in stadium vs. 5.34 otherwise).  In contrast, contiguous channel bonding performs worse in the stadium (3.69 in stadium vs. 5.19 otherwise) even under the same average load.  The reason may be the minimal inter-channel correlation at the stadium. Indeed, the stadium management confirmed that no channel bonding was implemented in any of the stadium's APs.

% \textit{Finding}: Even under the stadium's extremely high average load, short durations of lower load can be exploited to yield significant throughput gains.
